Union: A Unified HW-SW Co-Design Ecosystem in MLIR for Evaluating Tensor Operations on Spatial Accelerators

To meet the extreme compute demands for deep learning across commercial and scientific applications, dataflow accelerators are becoming increasingly popular. While these "domain-specific" accelerators are not fully programmable like CPUs and GPUs, they retain varying levels of flexibility with respect to data orchestration, i.e., dataflow and tiling optimizations to enhance efficiency. There are several challenges when designing new algorithms and mapping approaches to execute the algorithms for a target problem on new hardware. Previous works have addressed these challenges individually. To address this challenge as a whole, in this work, we present a HW-SW co-design ecosystem for spatial accelerators called Union within the popular MLIR compiler infrastructure. Our framework allows exploring different algorithms and their mappings on several accelerator cost models. Union also includes a plug-and-play library of accelerator cost models and mappers which can easily be extended. The algorithms and accelerator cost models are connected via a novel mapping abstraction that captures the map space of spatial accelerators which can be systematically pruned based on constraints from the hardware, workload, and mapper. We demonstrate the value of Union for the community with several case studies which examine offloading different tensor operations(CONV/GEMM/Tensor Contraction) on diverse accelerator architectures using different mapping schemes.

==> pact20_latex_template/6_related_works.tex <==
\section{Related Work}

\siva{I would remove this section, seems just an obligation. We covered related work before.}
In this section, we restrict our attention on two categories of prior work -- 1) Frameworks for evaluating accelerators, and 2) Abstractions used for describing algorithms (problems), mappings, and architecture descriptions.

We briefly described the comparison of our \UNION framework with prior frameworks in the Section~\ref{sec:background} and also in Table~\ref{comparision}.
Also, the comparison of our unified abstractions with prior abstractions are discussed in Section~\ref{sec:union_interface} (A) and (C).

% \subsection{HW-SW Co-Design Ecosystem}

% Because of higher performance required in deep learning, a lot of frameworks are emerging 

% \subsection{Abstractions}

% \subsection{Timeloop}
% Timeloop is composed of two main components: timeloop-mapper and timeloop-model.

% \subsection{TVM}
% TVM is a compiler which includes optimizations for deep learning workloads for various hardwares. Although they expose various optimization opportunities for CPUs and GPUs, they use VTA as their target accelerators.

% \subsection{Spatial}
% Koeplinger et al. introduced a language and compiler, Spatial~\cite{spatial_pldi18}, for high level descriptions of reconfigurable accelerators. 
% Their work focused on high-level synthesis language design of reconfigurable architectures with a number of optimizations. 
% They have not explored using different mappers and cost models, but instead used an active learning-based autotuner, HyperMapper as their mapper and a extended analytical model used in their previous work, Delite Hardware Definition Language.

% \subsection{Interstellar with Halide}


==> pact20_latex_template/algorithms/gemm.tex <==
\begin{algorithm}[t]
% \scriptsize
%\footnotesize
\SetInd{0.45em}{0.45em}
\SetAlgoLined
\DontPrintSemicolon
\KwIn{ \TODO{Fix here} \\
M = N = K = 32, GEMM with BF16 and FP 32 for input and output data types.
\\
}
%dataflow\_candidates $\leftarrow$ {\scriptsize \textbf{get\_candidate\_LoopOrders\_ClusterSzs}(\textit{Arch}, \textit{P})};\\
%\textit{num\_LoopOrders} $\leftarrow$ {\scriptsize \textbf{get\_num\_LoopOrders}(dataflow\_candidates)};\\ \textit{num\_ClusterSzs} $\leftarrow$ {\scriptsize \textbf{get\_num\_ClusterSzs}(dataflow\_candidates)};\\

% \textit{num\_LoopOrders} $\leftarrow$ dataflow\_candidates.shape[0]; \textit{num\_ClusterSzs} $\leftarrow$ dataflow\_candidates.shape[1];\\

% \Comment*[r]{\textbf{\textcolor{blue}{num\_LoopOrders = candidate\_dataflows.shape[0]}}}
% \Comment*[r]{\textbf{\textcolor{blue}{num\_ClusterSzs = candidate\_dataflows.shape[1]}}}
\vspace{5}

// load C Tiles to tmm registers \\
%tileloadd tmm0, ptr [rax+r11*4] \\
\textit{tileloadd} tmm0, ptr[CTile0]  \\
\textit{tileloadd} tmm1, ptr[CTile1] \\
\textit{tileloadd} tmm2, ptr[CTile2] \\
\textit{tileloadd} tmm3, ptr[CTile3] \\
\texttt{\\}
// Compute partial sums\\
\textit{tileloadd} tmm4 BTile0 \\
\textit{tileloadd} tmm6 ATile0 \\
\textit{tdpbf16ps} tmm0, tmm6, tmm4 \\
\textit{tileloadd} tmm5 BTile1 \\
\textit{tdpbf16ps} tmm2, tmm6, tmm5 \\
\textit{tileloadd} tmm7 ATile1 \\
\textit{tdpbf16ps} tmm1, tmm7, tmm4 \\
\textit{tdpbf16ps} tmm3, tmm7, tmm5 \\
\texttt{\\}
// store C Tiles to tmm registers \\
\textit{tilestored} ptr[CTile0], tmm0 \\ 
\textit{tilestored} ptr[CTile1], tmm1 \\
\textit{tilestored} ptr[CTile2], tmm2 \\
\textit{tilestored} ptr[CTile3], tmm3 \\

%tilestored ptr [r12+r14*4], tmm0


\caption{GEMM Example with AMX instructions}
\label{alg:flash_setup}
\end{algorithm}

==> pact20_latex_template/backup/intro.tex <==
\section{Introduction}



Deep Neural Networks (DNNs) have provided tremendous improvements over traditional methods and are widely employed in various domains, including, but not limited to, computer vision~\cite{resnet_cvpr16}, natural language processing~\cite{bert}, and recommendation~\cite{dlrm}. 
Their high computing requirements has motivated the development of specialized ASIC accelerators, both from industry and academia~\cite{tpu_isca17, eyeriss_isca16, maeri_asplos18}, as promising solutions to meet tight latency, throughput and energy requirements that CPUs and GPUs cannot provide.
%the Moore's law \roberto{not sure why we're bringing in the end of Moore's law, I guess the accelerators we're targeting are not quantum or neuromorphic, are they?}.
These accelerators usually deploy a number of Processing Elements (PEs) spatially  and improve the overall throughput by parallelizing the  executions of fundamental operations, such as Multiply-and-Accumulate for CNN workloads.
These accelerators minimize data movement by exploiting spatial, temporal, and spatio-temporal reuse forms for energy efficiency.
To do so, these accelerators design customized 
scratchpad buffer hierarchies and sophisticated Networks-on-Chip (NoC) to enable data reuse through the memory hierarchy or over wires (i.e., dataflow).
% recent accelerators leverage various fixed Network-on-Chip (NoC) designs which support multicast, broadcast, and peer to peer forwarding, and flexible NoCs for distributing and reducing data with custom memory hierarchy using scartchpads.

Because of the extreme diversity in deployment domains (IoT/ edge/ cloud), application domains (vision/ language/ recommendation/ scientific), 
and evolving algorithmic workload shapes, there is no ``one-size-fits-all'' design that can claim the best performance and energy efficiency across the landscape. Instead, many different hardware designs  with varying microarchitectures and flexibility are being actively researched and proposed to solve specific problems.
Many of these designs are re-configurable architectures and can adapt to varying workload within a certain degree.
On the other hand, this new ``cambrian era'' of computer architecture has produced a moltitude of novel hardware concepts. Further, many of these accelerators have been designed for very specific domains (e.g., AI) and are intended to programmed with domain-specific languages (DSLs) such as PyTorch. Comparing all those novel designs and understanding whether they provide a solution for a specific problem/workload has become incredibly difficult, especially in early stage when multiple design choices are still open. There is need of  generic framework for evaluating new spatial architectures and tensor kernels in a way tht is flexible, composable, and resusable across the hardware and software stack.
% Also, since DNN researchers keep proposing new DNN architecture with specialized tensor kernels, it is necessary to have a generic framework for evaluating new spatial architectures and tensor kernels.

Computer architects use simulators and analytical cost models to estimate the performance of new accelerators to minimize the design-to-test time and the the faster design space exploration.
Recent works have proposed analytical cost models~\cite{maestro_micro19, timeloop_ispass19} and simulators~\cite{scalesim_ispass20, stonne}. for evaluating spatial accelerators. 
Different cost models target a different set of accelerators. 
However, if one wants to explore different accelerators, he/she may need to switch to the different frameworks back and forth which introduces non-trivial engineering overhead due to the lack of an unified ecosystem for evaluating accelerators.
Moreover, users often need to re-implement benchmarks and kernels in a way that can be used to drive the framework, e.g., OpenMP, custom pragmas or languages, PyTorch, etc.
To wrap different cost models under a single umbrella to improve usability and modularity, 
there should be \emph{unified abstractions} which can be used across different cost models. 
For example, cost models usually take workload (problem), mapping (dataflow and tile sizes), and hardware description as the input files. 
To generate a workload file to use a cost model, either a user should translate the operator in a specific format for the cost model~\cite{timeloop_ispass19} or translate DNN models into smaller supported DNN operators such as CONV, FC, and Depth-wise CONV~\cite{maestro_micro19}. Since this process is different depending on the frameworks, it should be done manually which can be both error-prone and tedious. To get rid of this inefficiency, there should be a unified way of deriving a \textit{workload abstraction} for the cost model.

This problem is not limited to the workload file. Different cost models use their own mapping formats. For example, MAESTRO~\cite{maestro_micro19} introduced a new data-centric representation to describe the mapping, Interstellar~\cite{interstellar_asplos20} uses \TODO{todo}, Timeloop~\cite{timeloop_ispass19} uses compute-centric representation which is based on the classic loop nest, and so on. 
Without proper optimization from the compiler to determine the right mapping,
the performance of the hardware can degrade significantly as prior works have shown~\cite{timeloop}.
%the performance of the underlying hardware would result in significant reduction. 
This has motivated research in mappers~\cite{marvel, timeloop_ispass19, gamma_iccad20} to find efficient mappings on a target spatial architecture through various techniques including exhaustive search, random sampling, heuristic-based pruning, and genetic algorithm.
Marvel and GAMMA~\cite{gamma_iccad20} use MAESTRO~\cite{maestro_micro19} as their cost model while mappers implemented in Timeloop~\cite{timeloop_ispass19} and Interstellar~\cite{interstellar_asplos20} can only use the internal cost models in these tools.
The existing mappers~\cite{marvel, dmazerunner, gamma_iccad20, interstellar_asplos20, timeloop_ispass19}, which find an optimal mapping for the target workload and accelerator, are tightly dependent on their cost models due to the different representations.
This limits the interoperability and reusability of the mappers even though conceptually mappers could be used among different cost models if there is an \textit{unified mapping abstraction}.

%Due to their different input descriptions, MAESTRO can be used as a DSE tool for flexible accelerators like MAERI while Timeloop has strength for its hierarchical hardware descriptions supporting any perfectly nested loop nests as its inputs.
%Spatial architectures can be categorized into three categories: fixed, flexible, and multiple chiplets. Certain mappers/cost models can be used for a set of those accelerators, but none of them can be used for all categories. 



%In today’s evaluation, the DNN models are translated into a set of operators in customized formats and use their own optimizers and cost models to estimate the performance. 
%The challenges with this approach are 1) not able to leverage other exploration strategies or cost models 2) depending on manual translation from the DNN model into the custom formats which is error prone, Automatic -- different translators for different frameworks (This is where we are leveraging the efforts of MLIR).

%\geonhwa{@Gokcen, Please describe why we use MLIR here}
To solve the aforementioned issues, this work introduces \union. \union includes unified abstractions which can be used as an interface with different mappers and cost models (flexibility).
Then, we combine multiple different existing frameworks using the proposed abstractions (composability).
Our novel approach leverages the MLIR framework to connect  different high-level languages with multiple hardware back-ends. This approach enable us to re-use most of the intermediate layers (where most generic optimizations and transformations are performed) when changing the programming language and/or the hardware back-end (re-usabiliy).
MLIR is getting tremendous attention recently in compiler research due to its high re-usability and inter-operability with other software components, thus we foresee that our solution will be able to inter-operate with many programming languages, compilers, and computer architectures. We leverage MLIR for 1) getting unified workload description 2) operator-level analysis and transformation.


%


%Our framework can be used as either finding optimal mappings or exploring HW design space. 

To the best of our knowledge, \union is the first framework unifying multiple high level languages, mappers, and cost models for spatial accelerators leveraging MLIR. 
We believe that our work would reduce the burden of both computer architects, compiler researchers and domain experts by clearly decoupling the intermediate layers. In summary, the contributions of this paper are listed below: 

%\tushar{ 
%We explicitly expose the design-space and mapping space for the given problem on a certain target accelerator. , and role of compiler - mapper - HW DSE etc etc … so it becomes a paper to bring in all of this into one framework and so that’ll be the key contribution …}

\begin{itemize}
    \item We provide a plug-and-play unified infrastructure to combine high level applications such as ML and HPC, mappers, cost models of spatial accelerators.
    \item We design an interface to connect with different mappers and cost models with a new mapping abstraction which covers various existing mapping descriptions including both compute-centric and data-centric notations for spatial accelerators.
    \item We introduce operator-level/loop-level analysis to identify operators to be evaluated with the target spatial accelerator with a cost model.
    \item We show how our framework can be used in various workloads with different mappers and cost models for diverse set of accelerators, including flexible and chiplet-based. 
    %\item Evaluation: regular conv2d, conv3d... DSL for TC.. different accelerator configurations.. sparse kernels...Dense + Sparse workloads
\end{itemize}





==> pact20_latex_template/pact2021_information.tex <==
IMPORTANT DATES and DEADLINES

Conference Papers:
Abstracts: April 15, 2021
Full Papers: April 19, 2021
Round 1 Rebuttal Period: May 24-25, 2021
Round 2 Rebuttal Period: June 28-29, 2021
Author Notification: July 5, 2021
Artifact Submission: July 12, 2021
Camera Ready Papers: August 16, 2021

Workshops and Tutorials:
Proposals: April 26, 2021

For PACT 2021 we solicit contributions in a broad range of topics, including (but not limited to) the following:

o) Parallel architectures and computational models
o) Compilers and tools for parallel computing systems
o) Multicore, multithreaded, superscalar, and VLIW architectures
o) Software and hardware support for hiding memory latencies
o) Correctness and security issues in parallel hardware, software and tools
o) Reconfigurable parallel computing
o) Dynamic translation and optimization
o) I/O issues in parallel computing
o) Parallel programming languages
o) Execution environments and middleware for parallel computing
o) Application- and domain-specific parallel systems
o) Applications and experimental systems studies of parallel processing
o) Heterogeneous systems using various types of accelerators
o) Applications of machine learning to parallel computing
o) Future parallel systems for beyond Moore’s law and/or beyond Exascale
o) Computing systems aspects of parallel algorithms
o) Computing systems aspects of distributed and mobile computing
o) Computing systems insights from high-performance applications (including machine learning, data analytics, scientific computing, computational biology)

==> pact20_latex_template/tables/framework_comparisons.tex <==
% another column compiler ? standalone ?
\begin{table*}[t]
\caption{Comparison with existing frameworks for mapping tensor operators on spatial accelerators.\tushar{@prasanth - can you go through this table and help populate it -- see if you want to bring in other related works from Marvel paper. Should AutoTVM hw be VTA or generic accelerator?}}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Framework} & Supported operators & Target HW & Memory level& Cluster-centric & Cost models & Front-end & Mappers\\
\hline\hline
AutoSA~\cite{autosa} & Fully nested loops & Systolic Array & Fixed & No & Polyhedral & N/A \\
\hline
mRNA~\cite{mrna} & CONV2D & MAERI & Fixed & No & mRNA & N/A \\
\hline
AutoTVM & CONV2D, GEMM & Generic accelerator & Fixed & No & TVM & TVM \\
\hline
Interstellar~\cite{interstellar_asplos20} & CONV2D & Generic accelerator & Arbitrary & No & Interstellar & Halide \\
\hline
dMazeRunner~\cite{dmazerunner} & Fully nested loops & Generic accelerator & Fixed & No & dMazeRunner & TVM \\
\hline
Timeloop~\cite{timeloop_ispass19} & Fully nested loops & Generic accelerator & Arbitrary & No & Timeloop & N/A \\
\hline
Mind Mapping~\cite{mindmapping_asplos21} & Fully nested loops & Generic accelerator & Arbitrary & No & Timeloop & N/A  \\
\hline
GAMMA~\cite{gamma_iccad20} & CONV2D, GEMM & Generic accelerator & Fixed & Yes & MAESTRO & N/A \\
\hline
Marvel~\cite{marvel} & CONV2D, GEMM & Generic accelerator & Fixed & Yes & MAESTRO & N/A\\
\hline
\textbf{UNION} & \textbf{Fully nested loops} & \textbf{Generic accelerator} & \textbf{Arbitrary} & \textbf{Yes} &  \textbf{Multiple} & \textbf{MLIR}\\
\hline
%\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table*}
